Comprehension Is a Double-Edged Sword: Over-Interpreting Unspecified Information in Intelligible Machine Learning Explanations

Automated decision-making systems are becoming increasingly ubiquitous, which creates an immediate need for their interpretability and explainability. However, it remains unclear whether users know what insights an explanation offers and, more importantly, what information it lacks. To answer this question we conducted an online study with 200 participants, which allowed us to assess explainees' ability to realise explicated information -- i.e., factual insights conveyed by an explanation -- and unspecified information -- i.e, insights that are not communicated by an explanation -- across four representative explanation types: model architecture, decision surface visualisation, counterfactual explainability and feature importance. Our findings uncover that highly comprehensible explanations, e.g., feature importance and decision surface visualisation, are exceptionally susceptible to misinterpretation since users tend to infer spurious information that is outside of the scope of these explanations. Additionally, while the users gauge their confidence accurately with respect to the information explicated by these explanations, they tend to be overconfident when misinterpreting the explanations. Our work demonstrates that human comprehension can be a double-edged sword since highly accessible explanations may convince users of their truthfulness while possibly leading to various misinterpretations at the same time. Machine learning explanations should therefore carefully navigate the complex relation between their full scope and limitations to maximise understanding and curb misinterpretation.

==> table_matrix.tex <==
\todo[inline,caption={Table Notes}]{
Here's an explainer of what the entries in Table~\ref{tab:explainer_matrix} mean. When you get on with writing the paper, you will need to weave this information into the text. %
\begin{itemize}%
    \item \emph{model transparency} is a full and complete view -- this is a global explanation%
    \begin{itemize}
        \item for the decision tree you can put class proportions in the leaves to provide the explainee with a classification probability (since the logistic regression model outputs these as well)
        \item then $p(x) \in [0, 1]$
        \item and $f(x) = \text{survived}$ or $f(x) = \text{died}$
        \item the mathematical notation for decision trees is atrocious -- I think we should stick to tree visualisation
    \end{itemize}
    \item \emph{decision surface} -- this is a partial/incomplete explanation (because we are limited to two dimensions, we freeze all feature values but two and only show the change in the decision boundary for these two [again to 2-D visual counterfactuals]); it is local (encompasses a limited area)
    \begin{itemize}
        \item since the surface is local, we should probably just plot the one data point for which the surface was generated (i.e., the one whose feature values other than the ones displayed on the axes are frozen)
        \item these also capture 2-D \emph{individual feature dependence} (kind of \emph{individual conditional expectation}) because you can infer how a change in a given attribute (along the x-axis, y-axis, or both at the same time) influences the prediction
    \end{itemize}
    \item \emph{counterfactuals} -- these are explicitly local and can be based on any number of features (as opposed to the pseudo-counterfactuals captured by the decision surface, which can only be for up to 2 features)
    \begin{itemize}
        \item counterfactuals should be more informative for logistic regression than for decision tree since they are already encapsulated by the model transparency in the latter case
    \end{itemize}
    \item \emph{feature importance/influence}
    \begin{itemize}
        \item we have 2 types of feature importance: global and local
        \item we also have 2 ways to represent it: numerical and visual (bar chart)
        \item I'm not quite sure whether we should include both (and with what scope and in what modality)
        \item we can probably split it into \emph{influence} and \emph{importance} to make them distinguishable; in this case the \emph{global would be importance} and the \emph{local would be influence} -- this appears to make the most sense here
        \item then we need to decide on modality: influence can be numerical/bar chart/force; importance can be numerical/bar char -- \textbf{suggestions welcome} 
        \item \textbf{global feature importance} is calculated as follows: the absolute value of coefficients for the logistic regression (assuming that the features were normalised in the first place); the reduction in Gini impurity (provided by the learnt tree) for decision tree
        \item \textbf{local feature influence} is calculated as follows:
        \begin{itemize}
            \item the product of each feature value and its coefficient in the logistic regression equation for a particular data point (again, assuming that the features were normalised in the first place);
            \item for decision tree, the \emph{global feature importance} formula applied only to (tree splitting) nodes present on the path that is used to predict the selected instance; additionally, we need to make sure that the influence computer for a feature at each splitting node can be either negative or positive since the importance formula only gives positive values, which we can get by checking whether the probability (proportion of instances in the node) of the positive class (the desired outcome) increases or decreases between the two splitting nodes being compared (i.e., down the tree hierarchy)
        \end{itemize}
    \end{itemize}
\end{itemize}}%

\afterpage{%
    \clearpage%
    \begin{landscape}%
    \vspace*{\fill}
    \begin{table}[htb!]%
    \centering
    \caption{Overview of the predictive models and explainers used for the user study.\label{tab:explainer_matrix}}
    \begin{tabular}{@{}p{2.5cm} c p{3.4cm} p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}@{}}
    \toprule
    Model Type && \multicolumn{5}{c}{Explainability Approach} \\% Explainability Approach
    \cmidrule{3-7}
    && Model Transparency (global) & Decision Surface (visual, cohort/local) & Counterfactual (textual, local) & Feature Importance (numerical, global) & Feature Influence (visual [TBD: bar chart / force plot], local) \\% Mathematical Formulation
    \midrule
    Logistic Regression && %
            $ p(x) = \frac{1}{1 + e^{-(\omega_0 + \omega_1 x_1 + \cdots)}} $
            $ f(x) = \begin{cases}
                1 & \text{if} \;\; p(x) \geq 0.5\\
                0 & \text{else}
            \end{cases} $ &
            \raisebox{-0.75\height}{\includegraphics[width=2.45cm]{figures/dummies/logistic_regression_surface.png}} &
            {\em Had $x_1$ been $7$ instead of $42$, $x_4$ been $12$ instead of $3$ and $x_7$ been $3$ instead of $1$, the prediction would have changed.} &
\begin{tabular}{ll}
$x_1$ & $0.2$ \\
$x_2$ & $0.4$ \\
$x_3$ & $0.0$
\end{tabular} &
            \raisebox{-0.75\height}{\includegraphics[width=2.45cm]{figures/dummies/logistic_regression_influence.png}} \\% 
    Decision Tree && %
            \raisebox{-0.75\height}{\includegraphics[width=3.4cm]{figures/dummies/decision_tree.png}} %
            $f(x)=\sum_{i} \mathbbm{1} \{x \in N_i\} \times \overline{N_i}$
            &
            \raisebox{-0.75\height}{\includegraphics[width=2.45cm]{figures/dummies/decision_tree_surface.png}} &
            {\em Had $x_1$ been $7$ instead of $42$, $x_4$ been $12$ instead of $3$ and $x_7$ been $3$ instead of $1$, the prediction would have changed.} &
\begin{tabular}{ll}
$x_1$ & $0.2$ \\
$x_2$ & $0.4$ \\
$x_3$ & $0.0$
\end{tabular} &
            \raisebox{-0.75\height}{\includegraphics[width=2.45cm]{figures/dummies/decision_tree_influence.png}} \\% 
    \bottomrule
    \end{tabular}
    \end{table}
    \vspace*{\fill}
    \end{landscape}
    \clearpage%
}

